AURSAD: Universal Robot Screwdriving Anomaly Detection Dataset

Screwdriving is one of the most popular industrial processes. As such, it is increasingly common to automate that procedure by using various robots. Even though the automation increases the efficiency of the screwdriving process, if the process is not monitored correctly, faults may occur during operation, which can impact the effectiveness and quality of assembly. Machine Learning (ML) has the potential to detect those undesirable events and limit their impact. In order to do so, first a dataset that fully describes the operation of an industrial robot performing automated screwdriving must be available. This report describes a dataset created using a UR3e series robot and OnRobot Screwdriver. We create different scenarios and introduce 4 types of anomalies to the process while all available robot and screwdriver sensors are continuously recorded. The resulting data contains 2042 samples of normal and anomalous robot operation. Brief ML benchmarks using this data are also provided, showcasing the data's suitability and potential for further analysis and experimentation.

==> sections/notes.tex <==



When running the following script from the computer:

\begin{lstlisting}[language=Python]
sec myProg():
    write_output_float_register(25,modbus_get_signal_status("Shank_position",False))
end
myProg()
\end{lstlisting}

The shank position is updated. But if we create a program from the UR robot, and attempt to load and play it through the computer, it doesn't update the register output value. The script on the UR robot had the function defined as a primary program, since it could not be defined as a secondary using "sec". Because and error occured, saying the value isn't used in the program.



